Fighting Sampling Bias: A Framework for Training and Evaluating Credit Scoring Models

Scoring models support decision-making in financial institutions. Their estimation and evaluation are based on the data of previously accepted applicants with known repayment behavior. This creates sampling bias: the available labeled data offers a partial picture of the distribution of candidate borrowers, which the model is supposed to score. The paper addresses the adverse effect of sampling bias on model training and evaluation. To improve scorecard training, we propose bias-aware self-learning - a reject inference framework that augments the biased training data by inferring labels for selected rejected applications. For scorecard evaluation, we propose a Bayesian framework that extends standard accuracy measures to the biased setting and provides a reliable estimate of future scorecard performance. Extensive experiments on synthetic and real-world data confirm the superiority of our propositions over various benchmarks in predictive performance and profitability. By sensitivity analysis, we also identify boundary conditions affecting their performance. Notably, we leverage real-world data from a randomized controlled trial to assess the novel methodologies on holdout data that represent the true borrower population. Our findings confirm that reject inference is a difficult problem with modest potential to improve scorecard performance. Addressing sampling bias during scorecard evaluation is a much more promising route to improve scoring practices. For example, our results suggest a profit improvement of about eight percent, when using Bayesian evaluation to decide on acceptance rates.

==> algorithms/alg_acceptance_loop.tex <==
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetKwInOut{Return}{return}
\Input{distribution parameters $\BFmu_c^g, \BFmu_c^b, \BFSigma_c^g, \BFSigma_c^b, \delta_c, C$, sample sizes $n, h$, \textit{bad} ratio $b$, acceptance rate $\alpha$, number of iterations $j_{max}$, feature indicator $v$}
\Output{labeled accepts $D^a$, labeled rejects $D^r$, labeled holdout set $H$}

$D^* = \{(\BFX^*, \BFy^*)\} = \mbox{generate}(\BFmu_c^g, \BFmu_c^b, \BFSigma_c^g, \BFSigma_c^b, \delta_c, C, b, n)$  \tcp*[r]{generate data using Algorithm C.1}

$H = \{(\BFX^s, \BFy^s)\} = \mbox{generate}(\BFmu_c^g, \BFmu_c^b, \BFSigma_c^g, \BFSigma_c^b, \delta_c, C, b, h)$  \tcp*[r]{generate holdout set}

$\tau = (1-\alpha)$-th percentile of $x_v$ with respect to $D^*$ \tcp*[r]{simple business rule}

$D^a = \{(X^*_i, y^*_i) | x_{i, v} \geq \tau\}$ \tcp*[r]{accept $\alpha n$ applications}

$D^r = \{(X^*_i, y^*_i) | x_{i, v} < \tau\}$ \tcp*[r]{reject $(1 - \alpha) n$ applications}  


\For{$j \in \{1, 2, ..., j_{max}\}$}{

	$f_a(X)$ = accepts-based model trained over $D^a$ \;
	
	$f_o(X)$ = oracle model trained over $D^a \cup D^r$ \;
	
	$D_j = \{(\BFX, \BFy)\} = \mbox{generate}(\BFmu_c^g, \BFmu_c^b, \BFSigma_c^g, \BFSigma_c^b, \delta_c, C, b, n)$  \tcp*[r]{batch of new applications}
	
	$\tau = \alpha$-th percentile of $f_a(D_j)$ \tcp*[r]{compute acceptance threshold}
	
	$D_j^a = \{(X_i, y_i) | f_a(X_i) \leq \tau\}$ \tcp*[r]{accept $\alpha n$ applications}
	
	$D_j^r = \{(X_i, y_i) | f_a(X_i) > \tau\}$ \tcp*[r]{reject $(1 - \alpha) n$ applications}  
	
	$D^{a} = \bigcup\limits_{i=1}^j D^a_i$; $D^{r} = \bigcup\limits_{i=1}^j D^r_i$ \tcp*[r]{append accepts and rejects}
}

\Return{$D^a, D^r, H$}

==> algorithms/alg_basl.tex <==
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{labeled accepts $D^a = \{(\BFX^a, \BFy^a)\}$, unlabeled rejects $D^r = \{\BFX^r\}$, holdout set $H = \{\BFX^h\}$; meta-parameters: filtering ($\beta$), labeling ($\tau, \gamma, \theta$), stopping criteria ($j_{max}$, $\BFP(y^r|\BFX^r), \epsilon$)}
\Output{corrected scoring model $f_c(X)$}

$\BFX^r$ = filtering$(\BFX^a, \BFX^r, \beta)$ \tcp*[r]{filtering stage}  

$j = 0$; $V = \{\}$; $F = \{\}$  \tcp*[r]{initialization}  

\While{$(j \le j_{max})$ and $(\BFX^r \neq \emptyset)$ and $(V_j \geq V_{j-1})$}{

    $j = j + 1$
    
    $D^* = \{(\BFX^*, \BFy^*)\}$ = labeling$(D^a, D^r, \rho, \gamma, \theta)$ \tcp*[r]{labeling stage}  

    $D^a = D^a \cup D^*$ \tcp*[r]{append labeled rejects to the labeled sample}
    
    $\BFX^{r} = \BFX^{r} - \BFX^{*}$ \tcp*[r]{remove labeled rejects from the unlabeled sample}
	
	$F_j = f(X)$ = strong learner trained over augmented $D^a$  \tcp*[r]{training stage}  
	
    $V_j = \mbox{BM}(F_j, H, \BFP(y^r|X^r), \epsilon)$ \tcp*[r]{evaluate using a Bayesian metric}  
}

\Return{$f_c(X) = F_{\argmax(V)}$} \tcp*[r]{return best-performing strong learner}  

==> algorithms/alg_data_generation.tex <==
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetKwInOut{Return}{return}
\Input{distribution parameters $\BFmu_c^g, \BFmu_c^b, \BFSigma_c^g, \BFSigma_c^b, \delta_c, C$, sample size $n$, \textit{bad} ratio $b$}
\Output{labeled set of examples $D = \{(\BFX, \BFy)\}$}

$n_b = b n$; $n_g = n - n_b$ \tcp*[r]{compute class-specific sample sizes}  

$\BFX^g \sim  \sum_{c=1}^C \delta_c \mathcal{N}_k(\BFmu_c^g, \BFSigma_c^g)$ \tcp*[r]{generate $n_g$ good applications}  

$\BFX^b \sim  \sum_{c=1}^C \delta_c \mathcal{N}_k(\BFmu_c^b, \BFSigma_c^b)$ \tcp*[r]{generate $n_b$ bad applications}  

$\BFy^g = \vec{0}$; $\BFy^b = \vec{1}$  \tcp*[r]{define applications' labels}  

$D = \{(\BFX^g, \BFy^g) \cup (\BFX^b, \BFy^b)\}$  \tcp*[r]{construct a data set}  

\Return{$D$}

==> algorithms/alg_filtering_stage.tex <==
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetKwInOut{Return}{return}
\Input{accepts $\BFX^a$, rejects $\BFX^r$, meta-parameters $\beta = (\beta_l, \beta_u)$}
\Output{filtered rejects $\BFX^r$}

$g(X)$ = novelty detection algorithm trained over $\BFX^a$ \; 

$\BFs^r = g(\BFX^r)$ \tcp*[r]{predict similarity scores}

$\BFX^r = \{X_i \in \BFX^r| s^r_i \in \lbrack \beta_l, \beta_u \rbrack$ \}, $\beta_l$ and $\beta_u$ are percentiles of $\BFs^r$ \tcp*[r]{filter rejects}

\Return{$\BFX^r$}

==> algorithms/alg_labeling_stage.tex <==
\SetAlgoLined
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetKwInOut{Return}{return}
\Input{labeled accepts $D^a = \{(\BFX^a, \BFy^a)\}$, unlabeled rejects $D^r = \{\BFX^r\}$, meta-parameters $\rho, \gamma, \theta$}
\Output{selected labeled rejects $D^* = \{(\BFX^*, \BFy^*)\}$}

$\BFX^{*}$ = sample$(\BFX^r, \rho)$, $\rho$ is the sampling rate \tcp*[r]{random sample of rejects}  

$f(X)$ = weak learner trained over $\BFD^a$ \;        

$\BFs^* = f(\BFX^*)$ \tcp*[r]{score rejects with a weak learner}  

derive $c_g$: $\BFP(\BFs^* < c_g) = \gamma$, $\gamma$ is the percentile threshold \;

derive $c_b$: $\BFP(\BFs^* > c_b) = \gamma \theta$, $\theta$ is the imbalance parameter \;

$\BFX^{*} = \{X^*_i \in \BFX^* | s^*_i < c_g$ or $s^*_i > c_b$\} \tcp*[r]{select relevant examples}  

$\BFy^{*}: y_i^{*} = 0$ if $s^*_i < c_g$ and $y_i^{*} = 1$ if $s^*_i > c_b$ \tcp*[r]{assign labels}  

\Return{$\{(\BFX^*, \BFy^*)\}$}

==> tables/tab_app_autoencoder.tex <==
\begin{tabular}{@{\extracolsep{0pt}} llccccc}
    \hline
    \up \down Features & Sample & MMD & AUC & BS & PAUC & ABR \\ % & Rank \\
    \hline
    \up \down Raw & Accepts           & - & \textbf{.7984} (.0010) & \textbf{.1819} (.0004) & \textbf{.6919} (.0010) & \textbf{.2388} (.0019) \\ %  & \textbf{1.01} \\
    \hline
    \up Latent    & Accepts           & - & .7006 (.0034) & .2212 (.0008) & .6066 (.0026) & .3385 (.0023) \\ %  & 3.37 \\
    Latent        & Accepts + rejects & - & .7177 (.0020) & .2187 (.0004) & .6170 (.0013) & .3328 (.0024) \\ %  & 3.14  \\
    \down Latent  & Accepts + rejects & + & .7304 (.0011) & .2161 (.0004) & .6376 (.0019) & .3061 (.0036) \\ %  & 2.48 \\
    \hline
\end{tabular}


==> tables/tab_app_heckman.tex <==
\begin{tabular}{@{\extracolsep{0pt}} llccccccc}
    \hline
    \up \down 
    Approach & Classifier  & NF(S) & NF(O) & AUC & BS & PAUC & ABR \\
    \hline
    \up \down 
    Ignore bias & XGB & -- & 2,409 & .7984 (.0010) & .1819 (.0004) & .6919 (.0010) & .2388 (.0019) \\
    \hline
    \up \down
    Joint model & Bivariate probit   & 65    & 65    & .7444 (.0011) & .2124 (.0006) & .6397 (.0010) & .3018 (.0013) \\
    \hline
    \up
    Two-step & Probit + Probit & 60    & 61    & .7418 (.0011) & .2167 (.0006) & .6473 (.0010) & .3030 (.0017) \\
    Two-step & Probit + XGB    & 30    & 2,410 & \textbf{.8034} (.0011) & \textbf{.1828 }(.0004) & \textbf{.6934} (.0014) & \textbf{.2381} (.0019) \\
    \down
    Two-step & XGB + XGB       & 2,410 & 2,410 & .8027 (.0013) & .1843 (.0004) & .6887 (.0014) & .2473 (.0022) \\
    \hline
\end{tabular}

% \begin{tabular}{@{\extracolsep{1pt}} ccccccccc}
%     \hline
%     \up \down 
%     Selection & Outcome & NF (sel) & NF (out) & AUC & BS & PAUC & ABR \\
%     \hline
%     \up \down
%     \multicolumn{2}{l}{Bivariate probit} & 65 & 65 & .7444 (.0011) & .2124 (.0006) & .6397 (.0010) & .3018 (.0013) \\
%     \hline
%     \up 
%     Probit & Probit & 5   & 5   & .5872 (.0013) & .2632 (.0003) & .5646 (.0011) & .4497 (.0019) \\
%     Probit & Probit & 10  & 10  & .6974 (.0016) & .2551 (.0004) & .6178 (.0015) & .3466 (.0022) \\
%     Probit & Probit & 15  & 15  & .6953 (.0013) & .2635 (.0009) & .6120 (.0012) & .3609 (.0024) \\
%     Probit & Probit & 20  & 20  & .7166 (.0011) & .2434 (.0007) & .6316 (.0011) & .3219 (.0018) \\
%     Probit & Probit & 25  & 25  & .7182 (.0019) & .2390 (.0016) & .6214 (.0014) & .3324 (.0024) \\
%     Probit & Probit & 30  & 30  & .7203 (.0014) & .2364 (.0015) & .6219 (.0011) & .3321 (.0019) \\
%     Probit & Probit & 35  & 35  & .7140 (.0026) & .2344 (.0011) & .6240 (.0013) & .3310 (.0025) \\
%     Probit & Probit & 40  & 40  & .7194 (.0016) & .2272 (.0012) & .6222 (.0010) & .3352 (.0018) \\
%     Probit & Probit & 45  & 45  & .7263 (.0019) & .2227 (.0014) & .6315 (.0012) & .3248 (.0020) \\
%     Probit & Probit & 50  & 50  & .7400 (.0012) & .2166 (.0007) & .6436 (.0010) & .3068 (.0017) \\
%     Probit & Probit & 55  & 55  & .7408 (.0012) & .2172 (.0007) & .6450 (.0010) & .3041 (.0017) \\
%     \textbf{Probit} & \textbf{Probit} & \textbf{60}  & \textbf{60}  & \textbf{.7418} (.0011) & .2167 (.0006) & \textbf{.6473} (.0010) & \textbf{.3030} (.0017) \\
%     Probit & Probit & 65  & 65  & .7391 (.0012) & .2161 (.0007) & .6437 (.0011) & .3070 (.0018) \\
%     Probit & Probit & 70  & 70  & .7413 (.0012) & \textbf{.2144} (.0007) & .6445 (.0010) & .3039 (.0017) \\
%     Probit & Probit & 75  & 75  & .7346 (.0017) & .2227 (.0013) & .6267 (.0024) & .3131 (.0021) \\
%     Probit & Probit & 80  & 80  & .7347 (.0018) & .2223 (.0014) & .6257 (.0026) & .3133 (.0024) \\
%     Probit & Probit & 85  & 85  & .7326 (.0020) & .2210 (.0013) & .6250 (.0027) & .3165 (.0027) \\
%     Probit & Probit & 90  & 90  & .7361 (.0018) & .2201 (.0012) & .6256 (.0027) & .3164 (.0025) \\    
%     Probit & Probit & 95  & 95  & .7376 (.0016) & .2182 (.0010) & .6264 (.0027) & .3130 (.0023) \\    
%     \down
%     Probit & Probit & 100 & 100 & .7384 (.0016) & .2196 (.0012) & .6278 (.0025) & .3111 (.0022) \\    
%     \hline
%     \up
%     Probit & XGB & 5   & 2,410  & .8005 (.0011) & .1837 (.0004) & .6904 (.0013) & .2421 (.0020) \\
%     Probit & XGB & 10  & 2,410  & .8008 (.0012) & .1843 (.0004) & .6871 (.0013) & .2469 (.0019) \\
%     Probit & XGB & 15  & 2,410  & .8010 (.0011) & .1835 (.0004) & .6870 (.0013) & .2478 (.0018) \\
%     Probit & XGB & 20  & 2,410  & .8011 (.0012) & .1836 (.0004) & .6878 (.0014) & .2479 (.0019) \\
%     Probit & XGB & 25  & 2,410  & .8008 (.0012) & .1843 (.0004) & .6871 (.0013) & .2469 (.0019) \\
%     \textbf{Probit} & \textbf{XGB} & \textbf{30}  & \textbf{2,410}  & \textbf{.8034} (.0011) & \textbf{.1828} (.0004) & \textbf{.6934} (.0014) & \textbf{.2381} (.0019) \\
%     Probit & XGB & 35  & 2,410  & .8008 (.0011) & .1829 (.0005) & .6881 (.0014) & .2472 (.0019) \\
%     Probit & XGB & 40  & 2,410  & .8006 (.0012) & .1832 (.0005) & .6901 (.0014) & .2431 (.0021) \\
%     Probit & XGB & 45  & 2,410  & .8000 (.0011) & .1842 (.0004) & .6874 (.0013) & .2484 (.0019) \\
%     Probit & XGB & 50  & 2,410  & .8008 (.0012) & .1843 (.0004) & .6871 (.0013) & .2469 (.0019) \\
%     Probit & XGB & 55  & 2,410  & .8007 (.0011) & .1841 (.0004) & .6877 (.0013) & .2465 (.0019) \\
%     Probit & XGB & 60  & 2,410  & .8008 (.0012) & .1843 (.0004) & .6871 (.0013) & .2469 (.0019) \\
%     Probit & XGB & 65  & 2,410  & .8008 (.0012) & .1843 (.0004) & .6871 (.0013) & .2469 (.0019) \\
%     Probit & XGB & 70  & 2,410  & .8008 (.0012) & .1843 (.0004) & .6871 (.0013) & .2469 (.0019) \\
%     Probit & XGB & 75  & 2,410  & .8008 (.0012) & .1843 (.0004) & .6871 (.0013) & .2469 (.0019) \\
%     Probit & XGB & 80  & 2,410  & .8008 (.0012) & .1843 (.0004) & .6871 (.0013) & .2469 (.0019) \\
%     Probit & XGB & 85  & 2,410  & .8009 (.0012) & .1847 (.0004) & .6886 (.0014) & .2453 (.0021) \\
%     Probit & XGB & 90  & 2,410  & .8008 (.0012) & .1843 (.0004) & .6871 (.0013) & .2469 (.0019) \\    
%     Probit & XGB & 95  & 2,410  & .8008 (.0012) & .1843 (.0004) & .6871 (.0013) & .2469 (.0019) \\    
%     \down
%     Probit & XGB & 100 & 2,410  & .8008 (.0012) & .1843 (.0004) & .6871 (.0013) & .2469 (.0019) \\    
%     \hline
%     \up \down
%     XGB & XGB & 2,410 & 2,410 & .8027 (.0013) & .1843 (.0004) & .6887 (.0014) & .2473 (.0022) \\
%     \hline
% \end{tabular}


==> tables/tab_app_loeffler.tex <==
\begin{tabular}{@{\extracolsep{1pt}} lccccc}
    \hline
    \up \down 
    Estimator & No. features & AUC & BS & PAUC & ABR \\
    \hline
    \up 
    Logistic Regression    &  5   & .6782 (.0012) & .2611 (.0003) & .6017 (.0011) & .3611 (.0019) \\
    Logistic Regression    &  10  & .7034 (.0010) & .2482 (.0003) & .6234 (.0011) & .3310 (.0016) \\
    Logistic Regression    &  15  & .7090 (.0009) & .2459 (.0003) & .6261 (.0009) & .3278 (.0014) \\
    Logistic Regression    &  20  & .7181 (.0009) & .2362 (.0004) & .6346 (.0008) & .3138 (.0013) \\
    Logistic Regression    &  25  & .7212 (.0012) & .2327 (.0008) & .6231 (.0009) & .3274 (.0017) \\
    Logistic Regression    &  30  & .7218 (.0010) & .2309 (.0008) & .6239 (.0008) & .3244 (.0014) \\
    Logistic Regression    &  35  & .7146 (.0016) & .2299 (.0009) & .6236 (.0009) & .3277 (.0016) \\
    Logistic Regression    &  40  & .7242 (.0012) & .2266 (.0008) & .6255 (.0008) & .3255 (.0013) \\
    Logistic Regression    &  45  & .7307 (.0014) & .2222 (.0009) & .6351 (.0009) & .3155 (.0014) \\
    Logistic Regression    &  50  & .7417 (.0008) & .2169 (.0005) & .6445 (.0008) & .3021 (.0012) \\
    Logistic Regression    &  55  & .7416 (.0009) & .2167 (.0005) & .6445 (.0008) & .3019 (.0012) \\
    Logistic Regression    &  60  & .7423 (.0008) & .2160 (.0005) & .6468 (.0008) & .3000 (.0012) \\
    Logistic Regression    &  65  & .7415 (.0008) & .2252 (.0005) & .6461 (.0007) & .3005 (.0012) \\
    Logistic Regression    &  70  & .7432 (.0008) & .2143 (.0005) & .6467 (.0007) & .2991 (.0012) \\
    Logistic Regression    &  75  & .7352 (.0011) & .2218 (.0009) & .6268 (.0016) & .3094 (.0015) \\
    Logistic Regression    &  80  & .7356 (.0012) & .2217 (.0010) & .6264 (.0017) & .3087 (.0016) \\
    Logistic Regression    &  85  & .7360 (.0012) & .2204 (.0009) & .6276 (.0017) & .3088 (.0017) \\
    Logistic Regression    &  90  & .7368 (.0012) & .2195 (.0008) & .6262 (.0018) & .3118 (.0017) \\    
    Logistic Regression    &  95  & .7378 (.0011) & .2177 (.0007) & .6269 (.0018) & .3092 (.0016) \\    
    \down
    Logistic Regression    & 100 & .7386 (.0011) & .2171 (.0007) & .6276 (.0017) & .3084 (.0016) \\    
    \hline
    \up
    Bayesian Estimator &  5   & .6365 (.0011) & .2683 (.0002) & .5885 (.0007) & .3809 (.0014) \\
    Bayesian Estimator &  10  & .6215 (.0009) & .2605 (.0005) & .5434 (.0014) & .4487 (.0022) \\
    Bayesian Estimator &  15  & .6465 (.0015) & .2518 (.0008) & .5612 (.0013) & .4182 (.0024) \\
    Bayesian Estimator &  20  & .6515 (.0015) & .2515 (.0009) & .5719 (.0009) & .4048 (.0021) \\
    Bayesian Estimator &  25  & .6736 (.0013) & .2407 (.0007) & .5873 (.0010) & .3795 (.0016) \\
    Bayesian Estimator &  30  & .6774 (.0012) & .2390 (.0006) & .5924 (.0010) & .3729 (.0015) \\
    Bayesian Estimator &  35  & .6892 (.0014) & .2348 (.0008) & .5982 (.0011) & .3612 (.0016) \\
    Bayesian Estimator &  40  & .6906 (.0014) & .2314 (.0006) & .5978 (.0012) & .3637 (.0018) \\
    Bayesian Estimator &  45  & .6967 (.0013) & .2288 (.0004) & .5997 (.0013) & .3565 (.0018) \\
    Bayesian Estimator &  50  & .6977 (.0013) & .2294 (.0004) & .6002 (.0013) & .3561 (.0017) \\
    Bayesian Estimator &  55  & .7011 (.0010) & .2281 (.0003) & .6019 (.0012) & .3555 (.0016) \\
    Bayesian Estimator &  60  & .7006 (.0010) & .2273 (.0004) & .6028 (.0010) & .3540 (.0015) \\
    Bayesian Estimator &  65  & .7057 (.000/) & .2256 (.0003) & .6063 (.0009) & .3521 (.0014) \\
    Bayesian Estimator &  70  & .7072 (.000/) & .2252 (.0002) & .6085 (.0010) & .3499 (.0014) \\
    Bayesian Estimator &  75  & .7131 (.0008) & .2230 (.0002) & .6149 (.0008) & .3395 (.0013) \\
    Bayesian Estimator &  80  & .7149 (.0008) & .2215 (.0002) & .6150 (.0008) & .3373 (.0014) \\
    Bayesian Estimator &  85  & .7179 (.0007) & .2203 (.0002) & .6156 (.0010) & .3329 (.0014) \\
    Bayesian Estimator &  90  & .7186 (.0007) & .2200 (.0002) & .6142 (.0009) & .3348 (.0013) \\    
    Bayesian Estimator &  95  & .7196 (.0007) & .2199 (.0002) & .6144 (.0009) & .3341 (.0013) \\    
    \down
    Bayesian Estimator & 100 & .7208 (.0007) & .2192 (.0002) & .6158 (.0009) & .3327 (.0013) \\    
    \hline
\end{tabular}


==> tables/tab_app_reweighting.tex <==
\begin{tabular}{@{\extracolsep{0pt}} lllcccc}
    \hline
    \up \down Approach & Weights & Sample & AUC & BS & PAUC & ABR \\ %  & Rank \\
    \hline 
    \up \down No weights & -- & -- & .7984 (.0010) & .1819 (.0004) & .6919 (.0010) & .2388 (.0019) \\ %  & 5.21 \\
    \hline
    \up \multirow{4}{*}{Density ratio}   & KLIEP & Holdout    & .7930 (.0011) & .1874 (.0005) & .6815 (.0014) & .2543 (.0024) \\ %  & 8.52 \\
                                         & KLIEP & Validation & .7950 (.0011) & .1879 (.0005) & .6775 (.0013) & .2570 (.0023) \\ %  & 8.94 \\
                                         & LSIF  & Holdout    & .8033 (.0007) & \textbf{.1827} (.0004) & .6916 (.0013) & .2372 (.0021) \\ %  & 4.54 \\
    \down                                & LSIF  & Validation & .8027 (.0008) & .1837 (.0004) & .6936 (.0012) & .2365 (.0019)  \\ % & 4.58 \\
    \hline
    \up \multirow{4}{*}{Cluster-based}  & A/H & Holdout & .7979 (.0010) & .1861 (.0006) & .6895 (.0014) & .2447 (.0024) \\ %  & 6.68 \\
                                        & A/V & Holdout & .7988 (.0010) & .1863 (.0004) & .6848 (.0013) & .2473 (.0021) \\ %  & 7.20 \\
                                        & A/H & Validation & .8040 (.0008) & .1840 (.0004) & \textbf{.6961} (.0012) & \textbf{.2346} (.0022) \\ %  & \textbf{4.22} \\
    \down                               & A/V & Validation & .7955 (.0012) & .1844 (.0003) & .6884 (.0013) & .2407 (.0022)  \\ %  & 6.35 \\
    \hline
    \up \multirow{2}{*}{Isolation forest} & SS & Holdout    & \textbf{.8045} (.0009) & .1837 (.0004) & .6932 (.0013) & .2381 (.0021) \\ %  & 4.43 \\
    \down                                 & SS & Validation & .8029 (.0009) & .1845 (.0003) & .6925 (.0013) & .2407 (.0021) \\ %  & 5.33 \\
    \hline
\end{tabular}

==> tables/tab_feature_groups.tex <==
\begin{tabular}{@{\extracolsep{1pt}} lll}
    \hline
    \up \down 
    Group & No. features & Description \\
    \hline
    \up 
    G1 & 7    & Basic features describing the loan applicant \\
    G2 & 236  & G1 + loan parameters, applicant's attributes and financial data \\
    G3 & 296  & G2 + credit bureau data \\
    G4 & 692  & G3 + microgeographic data \\
    G5 & 787  & G4 + data on previous loan applications \\
    G6 & 2,117 & G5 + transactional bank data \\
    G7 & 2,327 & G6 + device data \\
    \down 
    G8 & 2,409 & G7 + online behavior data \\
    \hline
\end{tabular}


==> tables/tab_features.tex <==
\begin{tabular}{@{\extracolsep{1pt}} lll}
    \hline
    \up \down 
    Feature category & No. features & Feature examples \\
    \hline
    \up 
    Loan parameters            & 27   & Loan amount, loan duration, etc. \\
    Applicant's attributes     & 201  & Employment status, number of kids, etc. \\
    Applicant's financial data & 8    & Stated income, stated income per household member, etc. \\
    Credit bureau data         & 60   & Applicant's credit rating, etc. \\
    Microgeographic data       & 396  & Location of residence, residence type, etc. \\
    Previous loan applications & 95   & Number of previous loans, time since the last application, etc. \\
    Transactional bank data    & 1330 & Average monthly income, average monthly spendings, etc. \\
    Internet device data       & 210  & Device use to submit application, screen resolution, etc. \\
    \down 
    Online behavior data       & 82   & Time to fill out the application form, number of clicks, etc. \\
    \hline
\end{tabular}

==> tables/tab_lit_bias_correction.tex <==
\begin{tabular}{@{\extracolsep{0pt}} llllllll}
	\hline
	\up \down Reference & Method & Type & DP & TR & EV & MA & NT \\
	\hline
	\up
   \citet{blitzer_domain_2006}          & Structural correspondence learning  & RC & $\checkmark$ & & & $\checkmark$ & \\ 
   \citet{daume_iii_frustratingly_2009} & Supervised feature augmentation     & RC & $\checkmark$ & & & $\checkmark$ & \\ 
   \citet{saenko_adapting_2010}         & Supervised feature transformation   & RC & $\checkmark$ & & & $\checkmark$ & \\ 
   \citet{gopalan_domain_2011}          & Sampling geodesic flow              & RC & $\checkmark$ & & & $\checkmark$ & \\ 
   \citet{gong_geodesic_2012}           & Geodesic kernel flow                & RC & $\checkmark$ & & & $\checkmark$ & \\
   \citet{caseiro_beyond_2015}          & Unsupervised feature transformation & RC & $\checkmark$ & & & $\checkmark$ & \\
   \citet{satpal_domain_2007}           & Penalized feature selection         & RC & $\checkmark$ & & & $\checkmark$ & \\
   \citet{pan_domain_2011}              & Transfer component analysis         & RC & $\checkmark$ & & & $\checkmark$ & \\
   \citet{long_transfer_2014}           & Transfer joint matching             & RC & $\checkmark$ & & & $\checkmark$ & \\
   \citet{sun_return_2016}              & Correlation alignment               & RC & $\checkmark$ & & & $\checkmark$ & \\
   \citet{wang_extreme_2017}            & Extreme dimension reduction         & RC & $\checkmark$ & & & $\checkmark$ & \\ 
   \down \citet{atan_deep-treat_2018}   & Bias-removing autoencoder           & RC & $\checkmark$ & & & $\checkmark$ & \\
    \hline
    \up 
    \citet{heckman_sample_1979}              & Heckman's model                   & MB     &              & $\checkmark$ & &              & $\checkmark$ \\
    \citet{meng1985cost}                     & Heckman-style bivariate probit    & MB     &              & $\checkmark$ & &              & $\checkmark$ \\
   \citet{lin_support_2002}                  & Modified SVM                      & MB     &              & $\checkmark$ & &              &  $\checkmark$ \\ 
    \citet{daume_iii_domain_2006}        & Maximum entropy genre adaptation  & MB     &              & $\checkmark$ & &              & $\checkmark$ \\
    \citet{yang_adapting_2007}                & Adapt-SVM                         & MB     &              & $\checkmark$ & &              & $\checkmark$ \\
   \citet{marlin_collaborative_2009}                      & Multinomial mixture model         & MB     &              & $\checkmark$ & &              & $\checkmark$ \\ 
   \citet{bickel_discriminative_2009}        & Kernel logistic regression        & MB     &              & $\checkmark$ & &              & $\checkmark$ \\
    \citet{chen_co-training_2011}             & Co-training for domain adaptation & MB, RC & $\checkmark$ & $\checkmark$ & & $\checkmark$ & \\
    \citet{duan_domain_2012}                  & Domain adaptation machine         & MB     &              & $\checkmark$ & &              & $\checkmark$ \\
    \citet{long_adaptation_2014}              & Regularized least squares         & MB     &              & $\checkmark$ & &              & $\checkmark$ \\
   \citet{liu_robust_2014}                         & Robust bias-aware classifier      & MB     &              & $\checkmark$ & &              & $\checkmark$ \\
   \citet{joachims_unbiased_2016}            & Modified ranking SVM              & MB     &              & $\checkmark$ & &              & $\checkmark$ \\
   \citet{chen_robust_2016}                  & Robust bias-aware regression      & MB     &              & $\checkmark$ & &              & $\checkmark$ \\ 
   \citet{liu_kernel_2017}                   & Modified bias-aware classifier    & MB     &              & $\checkmark$ & &              & $\checkmark$ \\
    \down \citet{kugelgen_semi_2019}          & Semi-generative model             & MB     &              & $\checkmark$ & &              & $\checkmark$ \\
    \hline
    \up \citet{rosenbaum_central_1983}              & Model-based probabilities              & RW & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
   \citet{shimodaira_improving_2000}         & Distribution density ratios            & RW & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\ 
   \citet{zadrozny_learning_2004}            & Selection probabilities are known      & RW & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
    \citet{huang_correcting_2006}             & Kernel mean matching                   & RW & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
    \citet{cortes_sample_2008}                & Cluster-based frequencies              & RW & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
    \citet{sugiyama_direct_2008}              & Kullback-Leibler weights               & RW & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
    \down \citet{kanamori_least-squares_2009} & Least-squares importance fitting       & RW & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
   \citet{loog_nearest_2012}           & Nearest-neighbor based weights         & RW & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\ 
   \citet{gong_connecting_2013}        & Focusing on cases similar to test data & RW & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\ 
    \hline
    \up \citet{shimodaira_improving_2000} & Modified AIC                   & EM & & & $\checkmark$ & & $\checkmark$ \\
    \citet{sugiyama_subspace_2001}                & Subspace information criterion & EM & & & $\checkmark$ & & $\checkmark$ \\
    \citet{sugiyama_input-dependent_2006}        & Generalization error           & EM & & & $\checkmark$ & & $\checkmark$ \\
    \citet{sugiyama_covariate_2007}       & Importance-weighted validation & EF & & & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
    \down \cite{bruzzone_domain_2010}          & Circular evaluation strategy   & EF & & & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
	\hline
	\up \down \textbf{This paper} & \textbf{BASL and Bayesian evaluation} & \textbf{MB, EF} & & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
	\hline
\end{tabular}

==> tables/tab_lit_reject_inference.tex <==
\begin{tabular}{@{\extracolsep{1pt}} llccccl}
\hline
\up \down 
\multirow{2}{*}{Reference} & \multirow{2}{*}{Implemented technique(s)} & Training & Evaluation & Representative & Profit & \multirow{2}{*}{No. features} \\
 & & method(s) & method(s) & holdout sample & gains & \\
\hline
\up 
\citet{joanes_reject_1993}    & Reclassification                        & DA & -- &              &              & 3 \\
\citet{fogarty_multiple_2006} & Multiple imputation                     & DA & -- &              &              & 10 \\
\down 
\citet{xia_novel_2019}        & Outlier detection with isolation forest & DA & -- &              &              & 9 \\
\citet{liu2020new}            & Ensembling classifiers and clusteres    & MB & -- &              &              & 5, 23  \\
\citet{kang2021graph}         & Label spreading with oversampling       & DA & -- &              &              & 22  \\
\hline
\up 
\citet{boyes1989econometric}   & Heckman model variant (HM)           & MB & -- &              &              & 42  \\
\citet{feelders_credit_2000}   & Mixture modeling                     & MB & -- &              &              & 2  \\
\citet{chen_economic_2001}     & HM                                   & MB & -- & $\checkmark$ &              & 24 \\
\citet{banasik_sample_2003}    & HM                                   & MB & -- & $\checkmark$ &              & 30 \\
\citet{wu_handling_2007}       & HM                                   & MB & -- &              &              & 2  \\
\citet{kim_technology_2007}    & HM                                   & MB & -- & $\checkmark$ &              & 16 \\
\citet{chen_bound_2012}        & Bayesian model                       & MB & -- &              & $\checkmark$ & 40 \\
\citet{li_reject_2017}         & Semi-supervised SVM (S3VM)           & MB & -- &              &              & 7  \\
\citet{marshall_variable_2010} & HM                                   & MB & -- &              &              & 18 \\
\citet{tian_new_2018}          & Kernel-free fuzzy SVM                & MB & -- &              &              & 7, 14 \\
\citet{xia_rejection_2018}     & CPLE-LightGBM                        & MB & -- &              &              & 5, 17 \\
\citet{anderson_using_2019}    & Bayesian network                     & MB & -- &              &              & 7, 20 \\
\citet{kim_ensemble_2019}      & S3VM with label propagation          & MB & -- &              &              & 17 \\
\down 
\citet{shen2020three}          & Unsupervised transfer learning       & MB & -- &              &              & 20  \\
\hline
\up 
\citet{banasik_credit_2005}     & Banded weights                & RW     & -- & $\checkmark$ &              & 30 \\
\citet{verstraeten_impact_2005} & Resampling                    & RW     & -- & $\checkmark$ & $\checkmark$ & 45 \\
\down 
\citet{bucker_reject_2012}      & Missing data based weights & RW & -- &              &              & 40 \\
\hline
\up 
\citet{crook_does_2004}                & Banded weights, extrapolation    & RW, DA     & -- & $\checkmark$ &              & 30 \\
\citet{banasik_reject_2007}            & HM with banded weights           & MB, RW     & -- & $\checkmark$ &              & 30 \\
\citet{maldonado_semi-supervised_2010} & Self-learning, S3VM              & MB, DA     & -- &              &              & 2, 20, 21 \\
\citet{anderson_modified_2013}         & HCA, Mixture modeling            & DA, MB     & -- &              &              & 12 \\
\citet{nguyen_reject_2016}             & Parceling, HM, Banded weights    & DA, MB, RW & -- &              &              & 9  \\
\down 
\citet{mancisidor_deep_2020}           & Bayesian model, self-learning, S3VM & DA, MB & -- &              &              & 7, 58  \\
\hline
\up \down 
\textbf{This paper} & \textbf{BASL, Bayesian evaluation} & \textbf{DA} & \textbf{EF} & $\checkmark$ & $\checkmark$ & \textbf{2,410} \\ 
\hline
\end{tabular}

==> tables/tab_markets.tex <==
\begin{tabular}{@{\extracolsep{40pt}} llcc}
    \hline
    \up \down Parameter & Notation & (a) Microloans & (b) Installment loans \\
    \hline
    \up Acceptance rate      & $\alpha$ & $[.2, .4]$             & $[.1, .2]$                  \\
    Loan principal           & $A$      & $\$375$ (SD = $\$100$) & $\$17,100$ (SD = $\$1,000$) \\
    Total interest rate      & $i$      & $.1733$ (SD = $.01$)   & $.1036$ (SD = $.01$)        \\
    \down Loss given default & LGD      & $[0, 1]$               & $[0, 1]$                    \\
    \hline
\end{tabular}

==> tables/tab_params_methods.tex <==
\begin{tabular}{@{\extracolsep{0pt}} llll}
    \hline
    \up \down Bias correction method & Meta-parameter & Candidate values & Selected values \\
    \hline
    %\up \down Ignore rejects  & -- & -- & -- \\
    %\hline
    %\up \down Label all rejects as \textit{bad}  & -- & -- & -- \\
    %\hline
    \up \multirow{6}{*}{Bias-removing autoencoder} & Learning rate                  & .01                              & .01       \\
                                                   & Number of training epochs      & 50, 100                          & 100       \\
                                                   & Batch size                     & 50, 100                          & 100       \\
                                                   & Regularization parameter       & $10^{-1}, 10^{-2}, ..., 10^{-5}$ & $10^{-5}$ \\
                                                   & Number of hidden layers        & 3                                & 3         \\
    \down                                          & Bottleneck layer size          & .8$k$, $k$ is no. features       & .8$k$    \\
    \hline
    \up \down \multirow{2}{*}{Bivariate Heckman} & Number of features & 5, 10, ..., 100       & 65     \\
    \down                                        & Functional form    & probit, logit, linear & linear \\
    \hline
    \up \down \multirow{4}{*}{Two-Step Heckman}  & No. features (selection)    & 5, 10, ..., 2410       & 30     \\
                                                 & No. features (outcome)      & 5, 10, ..., 2410       & 2410   \\
                                                 & Functional form (selection) & Probit, XGB            & Probit \\
    \down                                        & Functional form (outcome)   & Probit, XGB            & XGB    \\

    \hline
    \up \multirow{2}{*}{Bureau score based labels} & Rating of \textit{good} risks & $\{AA\}, \{AA, A\}$ & $\{AA, A\}$ \\
    \down                                          & Rating of \textit{bad} risks  & $\{D\}, \{C, D\}$   & $\{D\}$     \\
    \hline
    \up \down Hard cutoff augmentation & Probability threshold & .3, .4, .5 & .5 \\
    \hline
    \up \multirow{4}{*}{Reweighting} & Truncation parameter      & .01, .05                   & .05 \\
                                     & Weight scaling            & yes,  no                   & yes \\
                                     & Density ratio estimation  & cluster-based, LSIF, KLIEP & cluster-based  \\
    \down                            & Number of leaves in DT    & 100                        & 100 \\
    \hline
    \up \multirow{2}{*}{Parceling} & Multiplier        & 1, 2, 3 & 1  \\
    \down                          & Number of batches & 10      & 10 \\
    \hline	
    \up \multirow{6}{*}{Doubly robust evaluation} & Truncation parameter        & .01, .05                   & .05 \\
                                                  & Weight scaling              & yes,  no                   & yes \\
                                                  & Density ratio estimation    & cluster-based, LSIF, KLIEP & cluster-based  \\
                                                  & Number of leaves in DT      & 100                        & 100 \\
                                                  & Reward prediction model     & LR, RF                     & RF \\
    \down                                         & Reward prediction threshold & $.1, .2, ..., .9$          & $.2$ \\
    \hline
    \up \multirow{5}{*}{Bias-aware self-learning} & Filtering thresholds $\beta$        & (0, 1), (.01, .99), (.01, 1) & (.01, 1) \\
	                                              & Sampling ratio $\rho$                & 1, .3                        & .3   \\
	                                              & Labeled percentage $\gamma$         & .01, .02, .03                & .01 \\
                                        	      & Imbalance parameter $\theta$        & 1, 2, 3                      & 2   \\
    \down                               	      & Max number of iterations $j_{max}$ & 5                             & 5   \\
    \hline
    \up \multirow{4}{*}{Bayesian evaluation} & Max number of trials $j_{min}$      & $10^2$, $10^3$, $10^4$ & $10^2$ \\
                                             & Max number of trials $j_{max}$      & $10^6$                 & $10^6$ \\
	                                         & Convergence threshold $\varepsilon$ & $10^{-6}$              & $10^{-6}$   \\
	                                         & Prior calibration                   & yes, no                & yes \\
    \hline
\end{tabular}

==> tables/tab_params_xgb.tex <==
\begin{tabular}{@{\extracolsep{26pt}} lccc}
    \hline
    \up 
    \multirow{2}{*}{Meta-parameter} & \multirow{2}{*}{Candidate values} & Selected values & Selected values \\
    \down
    & & (synthetic data) & (real data) \\
    \hline 
    \up Maximum number of trees & 100, 1,000, 10,000     & $100$             & 10,000 \\
    Early stopping rounds       & 100, no early stopping & no early stopping & $100$ \\
    Maximum depth               & $1, 3, 5$              & $3$               & $3$   \\
    Learning rate               & $.1, .3$               & $.1$              & $.1$   \\
    Bagging ratio               & $.8, .9, 1$            & $.8$              & $.8$  \\
    \down Feature ratio         & $.8, .9, 1$            & $.8$              & $.8$  \\
    \hline
\end{tabular}

==> tables/tab_results_ablation.tex <==
\begin{tabular}{@{\extracolsep{0pt}} lccccc}
    \hline
    \up \down Framework extension & AUC & BS & PAUC & ABR & Rank \\
    \hline 
    \up 
    Traditional self-learning              & .8059 (.0010) & .1804 (.0004) & .6868 (.0011) & .2387 (.0020) & 4.80 \\
    Filter rejects using isolation forest  & .8054 (.0011) & .1790 (.0004) & .6981 (.0013) & .2312 (.0022) & 3.93 \\
    Label rejects with a weak learner      & .8134 (.0006) & .1774 (.0002) & .6992 (.0009) & .2294 (.0011) & 3.60 \\
    Introduce the imbalance multiplier     & .8133 (.0006) & .1796 (.0002) & .7026 (.0010) & .2238 (.0012) & 3.48 \\
    Sampling rejects at each iteration     & .8157 (.0006) & .1765 (.0002) & .7035 (.0010) & .2254 (.0013) & 2.85 \\
    \down 
    Bayesian framework for early stopping  & \textbf{.8166} (.0007) & \textbf{.1761} (.0003) & \textbf{.7075} (.0011) & \textbf{.2211} (.0012) & \textbf{2.34} \\
    \hline
\end{tabular}

==> tables/tab_results_sim_exp1.tex <==
\begin{tabular}{@{\extracolsep{33pt}} llccc}
    \hline
    \up \down 
    Evaluation method & Metric & Bias & Variance & RMSE \\
    \hline 
    \up 
    Accepts-based evaluation & \multirow{2}{*}{AUC}  & $.1923$ & $.0461$ & $.2205$ \\
    \down Bayesian framework &                       & $.0910$ & $.0001$ & $.1000$ \\
    \hline
    \up Accepts-based evaluation & \multirow{2}{*}{BS}   & $.0748$ & $.0006$ & $.0828$ \\
    \down Bayesian framework     &                       & $.0038$ & $.0009$ & $.0566$ \\
    \hline
    \up Accepts-based evaluation & \multirow{2}{*}{PAUC} & $.2683$ & $.0401$ & $.2803$ \\
    \down Bayesian framework     &                       & $.1102$ & $.0002$ & $.1187$ \\
    \hline
    \up Accepts-based evaluation & \multirow{2}{*}{ABR}  & $.1956$ & $.0004$ & $.2010$ \\
    \down Bayesian framework     &                       & $.0039$ & $.0040$ & $.0929$ \\
    \hline
\end{tabular}

==> tables/tab_results_sim_exp2.tex <==
\begin{tabular}{@{\extracolsep{100pt}} lcc}
    \hline
    \up \down 
    Metric & Loss due to bias & Gain from BASL \\
    \hline 
    \up 
    AUC   & $.0591$ & $35.72\%$ \\
    BS    & $.0432$ & $29.29\%$ \\
    PAUC  & $.0535$ & $22.42\%$ \\
    \down 
    ABR   & $.0598$ & $24.82\%$ \\
    \hline
    \up \down 
    MMD  & $.5737$ & $3.74\%$ \\
    \hline
\end{tabular}
